Register transducers are marble transducers

Deterministic two-way transducers define the class of regular functions from words to words. Alur and Cern\'y introduced an equivalent model of transducers with registers called copyless streaming string transducers. In this paper, we drop the "copyless" restriction on these machines and show that they are equivalent to two-way transducers enhanced with the ability to drop marks, named "marbles", on the input. We relate the maximal number of marbles used with the amount of register copies performed by the streaming string transducer. Finally, we show that the class membership problems associated with these models are decidable. Our results can be interpreted in terms of program optimization for simple recursive and iterative programs.

==> Marbles arXiv/parts/bounded.tex <==
\label{sec:bounded}

A natural restriction of our marble transducers is to bound the number of marbles that can be simultaneously present in the stack. Indeed, if a machine uses at most $k$ marbles, it has $\mc{O}(|w|^{k+1})$ possible configurations on input $w$. As a consequence, \emph{it performs its computation in polynomial time}, and the function $f$ it computes is such that $|f(w)|= \mc{O}(|w|^{k+1})$. In particular, the exponential behaviors of Example \ref{ex:expo:mt} are no longer possible.

\begin{definition} A \emph{$k$-marble transducer} is a marble transducer such that every accessible configuration (i.e. reachable from the initial configuration) has a stack of at most $k$ marbles.
\end{definition}

This definition is semantical, but it can easily be described in a syntactical way
by storing the (bounded) number of marbles that are currently dropped on the
input.

\begin{remark} $0$-marble transducers are exactly two-way transducers. 
\end{remark}

As special instances of $1$-marble transducers we get programs with $2$ nested
for loops of shape \verb?for i in {1,...,|w|} ( for j in {1,...,i} (...)  )?.
Indeed, the outer index $i$ corresponds to the marble, and the inner $j$ to the
reading head that cannot move on the right of $i$.  However, this interpretation
does not take the two-way moves into account.


\begin{example} \label{ex:mul}Consider the function $\mul: w \# 0^n \mapsto (w\#)^n$ that produces $n$ copies of $w\#$. It can be realized by a $1$-marble transducer that successively drops the marble from first to last $0$, and each time scans and outputs $w\#$.
\end{example}

\begin{remark} For a $k$-marble transducer, it is enough to have one marble color. Indeed, the colors of the marbles dropped form a finite information that can be encoded in the states.
\end{remark}






The correspondence given by Theorem \ref{theo:sstmt} does not take the number of
marbles into account.  In particular, it does not produce a copyless $\SST$ if
we begin with a $0$-marble transducer.  We shall now give a more precise statement
that relates the maximal number of marbles to the number of "copy layers" in the
$\SST$, as defined below.




\begin{definition} \label{def:ksst}

An $\SST$ $(A,B, Q, \regs,q_0, \iota, \delta,\lambda,F)$ is said to be $k$-\emph{layered} if $\regs$ has a partition of the form $\regs_0, \dots, \regs_k$, such that $\forall q \in Q$, $\forall a \in A$, the following are true:

\item

\begin{itemize}

\item $\forall 0 \le i \le k$, only registers from $\regs_0, \dots, \regs_i$ appear in $\{\lambda(q,a)(x) \mid {x \in \regs_i}\}$;

\item $\forall 0 \le i \le k$, each register $y \in \regs_i$ appears at most once in $\{\lambda(q,a)(x) \mid  x \in \regs_i\}$.

\end{itemize}

\end{definition}

Note that $0$-layered $\SSTs$ are exactly copyless $\SSTs$ (only the second
condition is useful).  For $k \ge 1$, Definition \ref{def:ksst} forces each layer
$\regs_i$ to be "copyless in itself", but it can do many copies of deeper
layers ($\regs_j$ for $j<i$).  This update mechanism is depicted in Figure
\ref{fig:ksst} below; it mainly avoids copying twice a register in itself.

\begin{figure}[h!]

\begin{center}
\begin{tikzpicture}[scale=1]
	\node[] (in) at (-2.5,0) [above,right]{\small Input word};
	\node[above] (in) at (0,-0.2) []{ $b$};
	\node[above] (in) at (1,-0.2) []{  $a$};
	\node[above] (in) at (2,-0.2) []{  $b$};
	\node[above] (in) at (3,-0.2) []{  $b$};
	\node[above] (in) at (4,-0.2) []{  $b$};
	\node[above] (in) at (5,-0.2) []{  $a$};
	\draw[->] (0,-0.5) -- (2.8,-0.5);
	\draw[->] (0,-1) -- (2.8,-1);
	\draw[->] (0,-1.5) -- (2.8,-1.5);
	
	\draw[->,gray,dashed,thick] (3.2,-0.5) -- (3.8,-0.5);
	\draw[->,gray,dashed,thick] (3.2,-1) -- (3.8,-1);
	\draw[->,gray,thick] (3.2,-1) -- (3.8,-0.6);
	\draw[->,gray,dashed,thick] (3.2,-1.5) -- (3.8,-1.5);
	\draw[->,gray,thick] (3.2,-1.5) -- (3.8,-1.1);
	\draw[->,gray,thick] (3.2,-1.5) .. controls (4.5,-3) and (5,-0.5) .. (4.2,-0.5);
	
	\node[] (in) at (3,-0.5) []{\footnotesize $\regs_2$};
	\node[] (in) at (3,-1) []{\footnotesize $\regs_1$};
	\node[] (in) at (3,-1.5) []{\footnotesize $\regs_0$};
	\node[gray] (in) at (4,-0.5) []{\footnotesize $\regs_2$};
	\node[gray] (in) at (4,-1) []{\footnotesize $\regs_1$};
	\node[gray] (in) at (4,-1.5) []{\footnotesize $\regs_0$};
       \end{tikzpicture}
\end{center}
\vspace*{-1.4cm}
\caption{\label{fig:ksst} Update of the registers in a $2$-layered $\SST$}
\vspace*{-0.3cm}
\end{figure}

\begin{example} 
  The function $\mul:w \# 0^n \mapsto (w\#)^n$ (Example \ref{ex:mul}) can be
  computed by a 1-layered $\SST$ with $\regs_0 = \{x\}$ and $\regs_1 = \{y\}$ as
  follows.  First, when reading $w\#$, it stores $w\#$ in $x$, while keeping
  $\varepsilon$ in $y$.  Then, each time it sees a $0$, it applies $x \mapsto x,
  y \mapsto xy$.
\end{example}

We now provide a fine-grained correspondence between marbles and registers. Our result indeed extends Theorem \ref{theo:alur}, which corresponds to the case $k=0$.

\begin{theorem} \label{theo:kmtksst} 
  For all $k \ge 0$, $k$-marble transducers and $k$-layered $\SSTs$ describe the
  same class of functions.  The right to left conversion is effective in
  $\PTIME$.
\end{theorem}

\begin{proof}[Proof sketch.] 
  To convert a $k$-layered $\SST$ in a $k$-marble transducer, we adapt the
  transformation of Theorem \ref{theo:sstmt} in order to use no more than $k$
  marbles.  The idea is to write only the recursive calls that correspond to the
  copy of a register, the others being kept implicitly.  The $\PTIME$ complexity
  is obtained by adapting the construction of \cite{dartois2017reversible}.  For
  the converse implication, we first transform the $k$-marble transducer in an
  $\SST$ using \mbox{Theorem \ref{theo:sstmt}}.  Since the function $f$ computed
  by this $\SST$ is such that $|f(w)| = \mc{O}(|w|^{k+1})$, we use \mbox{Lemmas
  \ref{lem:boundedcopy}} and \ref{lem:kbounded} in order to build a $k$-layered
  $\SST$ for $f$.  A large amount of additional work is required to obtain these
  results, and it is the purpose of Section \ref{sec:membership}.
\end{proof}







==> Marbles arXiv/parts/conclusion.tex <==
We presented in this paper a new correspondence between $\SSTs$ and marble
transducers.  Showing that two models are equivalent is always interesting in
itself, but our result also provides a deeper understanding of their behaviors.
Indeed, it relates recursive and iterative programs (marbles) to streaming
algorithms ($\SSTs$), which are suitable for program optimization problems.
Since the equivalence problem is decidable for $\SSTs$ \cite{filiot2017copyful},
we also obtain for free that it is the case for marble transducers (which was not
previously known).

Note that our model is not closed under composition. It is the case for obvious asymptotic growth reasons, since marble transducers can compute one exponential ($\pow : a^n \mapsto a^{2^n}$) but not two of them ($\pow \circ \pow$). More surprisingly, there exist polynomial-size compositions that cannot be expressed by our transducers, as shown below.

\begin{claim} $\mul : w \#0^n \mapsto (w\#)^n$ is computable by an $\SST$, but not $0^n\#w \mapsto (w\#)^n$.
\end{claim}
This result mainly comes because marbles and $\SSTs$ give an \emph{orientation} on the input: we stack marbles "on the right", and the $\SST$ is a streaming process "from left to right".


\subparagraph*{Marbles and pebbles.} A non-oriented generalization of $k$-marbles, named \emph{$k$-pebble transducers} \cite{bojanczyk2018polyregular}, has recently been investigated in detail. In this case, the reading head is allowed to move on the right of a mark without lifting it, while keeping a stack discipline. The typical example of function computable with $1$ pebble is $\sq : A \rightarrow A \uplus \{\overline{a}\mid a \in A\}, abc \mapsto \overline{a}bc a \overline{b}c ab \overline{c}$, which associates to $w$ the concatenation with $|w|$ copies of itself, the $i$-th copy having its $i$-th letter overlined. This function cannot be computed by a marble transducer.

In \cite{lhote2020pebble}, the membership problem is solved for the classes of $k$-pebble transducers. Despite their similarity, neither their result (Theorem \ref{theo:nathan} below) nor our \mbox{Proposition \ref{prop:growth}} imply each other, and the proof techniques are significantly different. Indeed we consider different classes of functions, ours being designed for streaming implementations, but not theirs. The relationship between marbles and pebbles is depicted in Figure \ref{fig:conclu}.

\begin{theorem}[\cite{lhote2020pebble}] \label{theo:nathan} A function $f$ described by a $k$-pebble transducer is computable by an $\ell$-pebble transducer if and only if $|f(w)| = \mc{O}(|w|^{\ell+1})$ (and this property is decidable).
\end{theorem}

Contrary to us, they do not obtain tight asymptotic bounds. Furthermore, they only consider machines with a bounded number of marks, i.e. no exponential growths.



\begin{figure}[h!]

    \def\acircle{(0,0) circle (1)}
    \def\bcircle{(0,0.8) circle (1.8)}
    \def\ccircle{(0,1.6) circle (2.6)}
    \def\mcircle{(6.32,-1.5) circle (7.5)}
    \def\icircle{(0,2.4) circle (3.4)}
    
    	\begin{center}
	\hspace*{-0.4cm}
        \begin{tikzpicture}{scale=0.9}

	   % Remplissage rose
            \fill[red!15] \acircle;     
            \fill[red!15] {(2.8,4.7) circle (1.5)};

            
            \begin{scope}
            \clip {(0,-1) rectangle (8,2)};
            \fill[red!15] \icircle;
            \end{scope}
            
            \fill[red!15] (-0.94,0.37) -- (1.404,5.25) -- (4.246,4.3) -- (3.25,1.4) -- cycle;

            \draw \acircle node {$\substack{\textcolor{blue}{0\text{-pebble}} \\ =\\ \textcolor{red}{0\text{-marble}} \\ = \\ \textcolor{red}{0\text{-layered } \SST}}$};
            \draw \bcircle ;
            \draw \ccircle;
            \draw[dashed] \icircle;
            
            \draw[blue,dotted,thick] (0,4.7) -- (0,5.25);
             \draw[red,dotted,thick] (2.5,3.1) -- (2.7,3.6);
            
            \node at (0.8,1.5) {\textcolor{red}{$\substack{1\text{-marble} \\ = \\ 1\text{-layered } \SST}$}};
            \node at (-0.95,1.6) {$\substack{\textcolor{blue}{1\text{-pebble}}}$};
            
             \node at (0,0.86) {\tiny $\mc{O}(n)$};
             \node at (0,2.45) {\tiny $\mc{O}(n^2)$};
             \node at (0,4.05) {\tiny $\mc{O}(n^3)$};
             \node at (0,5.63) {\tiny $\cup_k \mc{O}(n^k)$};
            
            \node at (1.4,2.9) {\textcolor{red}{$\substack{2\text{-marble} \\ = \\ 2\text{-layered } \SST}$}};
            \node at (-1.2,3.1) {$\substack{\textcolor{blue}{2\text{-pebble}}}$};
            \node at (-1.4,4.5) {$\substack{\textcolor{blue}{\bigcup_{k} k\text{-pebble}}}$};
            \node at (2,4.15) {$\substack{\textcolor{red}{\bigcup_{k} k\text{-marble}}}$};
            
            
            \node at (3,5.2) {\textcolor{red}{$\substack{\text{marbles} \\ = \\ \SST}$}};
             \node at (2.9,6.04) {\tiny $2^{\mc{O}(n)}$};
             
             
             \fill[gray!110] {(0.8,0) circle (0.05)};
             \draw[gray,dotted,thick] (0.8,0) -- (6,0);
             \node[right] at (6.1,0.05) {\small \textcolor{gray}{$\mirror: abac \mapsto caba$}};
             
             \fill[gray!110] {(1.2,1) circle (0.05)};
             \draw[gray,dotted,thick] (1.2,1) -- (6,1);
             \node[right] at (6.1,1.05) {\small \textcolor{gray}{$\mul: w\#0^n \mapsto (w\#)^n$}};
             
             
             \fill[gray!110] {(-0.7,2) circle (0.05)};
             \draw[gray,dotted,thick] (-0.7,2) -- (6,2);
             \node[right] at (6.1,2.05) {\small \textcolor{gray}{$\sq: abc \mapsto \overline{a}bc a \overline{b}c ab \overline{c}$}};
             
             
            \fill[gray!110] {(1,3.75) circle (0.05)};
             \draw[gray,dotted,thick] (1,3.75) -- (6,3.75);
             \node[right] at (6.1,3.8) {\small \textcolor{gray}{$\powo^3: a^n \mapsto a^{n^3}$}};
             
             \fill[gray!110] {(3.5,5.7) circle (0.05)};
             \draw[gray,dotted,thick] (3.5,5.7) -- (6,5.7);
             \node[right] at (6.1,5.75) {\small \textcolor{gray}{$\pow: a^n \mapsto a^{2^n}$}};

        \end{tikzpicture}
        \end{center}
        
    \caption{\label{fig:conclu} Classes of functions studied in this paper (\textcolor{red}{red}) and in \cite{lhote2020pebble}{} (\textcolor{blue}{blue}).}
\end{figure}







\subparagraph*{Future work.} Our work opens the way to a finer study of the classes of functions described by marble and pebble transducers. The \emph{membership problem from $k$-pebble to $k$-marble} is worth being studied to complete the decidability picture. It reformulates as follows: given a function computed by a pebble transducer, can we implement it in streaming way? The answer seems to rely on combinatorial properties of the output. Another perspective is to define a \emph{logical description} of our transducers, which allows to specify their behavior in a non-operational fashion. No formalism is known for marble transducers, but it is known since \cite{engelfriet2001mso} that two-way transducers correspond to \emph{monadic-second-order transductions}. On the other hand, \cite{droste2019aperiodic} studies in detail a \emph{weighted logics} which describes the functions computed by weighted automata. Using proof techniques which are similar to ours, they relate the asymptotic growth of the function to the logical connectors required to describe it.










==> Marbles arXiv/parts/intro.tex <==




Regular languages have been a cornerstone of theoretical computer science since the 1950's. They can be described by several equivalent models such as deterministic, non-deterministic, or two-way (the reading head can move in two directions) finite automata \cite{shepherdson1959reduction}.

A natural extension consists in adding an output mechanism to finite automata.
Such machines, called \emph{transducers}, describe functions from words to words
(or relations when non-deterministic).  In this case, the landscape generally
becomes more complex, as noted in 1967 by D. Scott: \flqq{} the functions
computed by the various machines are more important - or at least more basic -
than the sets accepted by these device \frqq{} \cite{scott1967some}.
Furthermore, transducers provide a natural way to model simple programs that
produce outputs.


\subparagraph*{Regular functions and copyless register transducers.} The
particular model of \emph{two-way transducer} consists in a two-way automaton
enhanced with an output function.  It describes the class of \emph{regular
functions} which has been intensively studied for its natural properties:
closure under composition \cite{chytil1977serial}, logical characterization by
monadic second-order transductions \cite{engelfriet2001mso}, decidable
equivalence problem \cite{gurari1982equivalence}, etc.

In \cite{alur2010expressiveness}, the equivalent model of \emph{copyless
streaming string transducer} ($\SST$) is described.  This machine processes its
input in a one-way fashion, while storing pieces of their output in a finite set
of registers: it is at the same time simpler (since it reads the input only
once) and more complex (since it needs registers) than a two-way transducer.
Registers are updated by simple concatenation operations.  However, the content
of a register can never be duplicated ("copyless"), which allows one to
implement the model efficiently for a streaming use.

\subparagraph*{Copyful register transducers.} Regular functions remain quite
limited in terms of expressiveness, since the size of the output can be at most
linear in the input's.  In this paper, we study the class of functions computed
by copyful $\SSTs$, i.e. register transducers that can duplicate their registers.
With this model, it becomes possible to produce outputs that have a polynomial,
or even exponential, size in the input's.  Meanwhile, it preserves many "good
properties" of regular functions, such as decidability of the equivalence
problem \cite{filiot2017copyful}.


\subparagraph*{Marble transducers.} Our first objective is to extend the
aforementioned correspondence between copyless $\SSTs$ and two-way transducers,
by providing a model of transducer without registers that is equivalent to
copyful $\SSTs$.  For this, we define \emph{marble transducers} (introduced for
trees in \cite{engelfriet1999trips}) and show equivalence.  This model consists
in a two-way transducer that can drop several marks ("marbles") on its input,
following a stack discipline.  Indeed, new marbles can only be dropped on the
left of the positions already marked.  Informally, our result shows that copyful
$\SSTs$ correspond to some recursive algorithms (hence the stack).

A very natural way to restrict the power of marble transducers is to bound the number of marks that can be used. We define \emph{$k$-marble transducer} that can use at most $k$ marks. Intuitively, it corresponds to iterative algorithms with "for" loops, such that the maximal depth of nested loops is $k+1$. In particular, $0$-marble transducers are exactly two-way transducers (since they use no marbles). Whereas marble transducers in general can have an exponential execution time, a $k$-marble transducer runs in polynomial time, more precisely $\mc{O}(n^{k+1})$ when $n$ is the input's length. Hence, it produces outputs of size $\mc{O}(n^{k+1})$.

As a second main result, we show that \emph{$k$-marble transducers} are
equivalent to a model of \emph{$k$-layered \SSTs}, i.e. $\SSTs$ with hierarchical
restrictions on their copies.  In particular for $k=0$, we recover the
correspondence between two-way transducers and copyless $\SSTs$.

\subparagraph*{Optimization and class membership problems.} As evoked above, our models of marble transducers have at most an exponential complexity (or "execution time"), but it becomes polynomial if we restrict the number of marks used. In practice, a natural question is that of optimization: can we transform an exponential algorithm in a polynomial equivalent one? Can we reach the smallest possible complexity? Having a tool to optimize programs is of foremost interest since it allows to write naive algorithms without worrying about the complexity. Due to well-known undecidability statements, optimizing any algorithm is hopeless in theory, thus having results for a "regular" kernel is already interesting. 

From a theoretical point of view, the optimization problem is known as
(effective) \emph{class membership problem}.  It instantiates as follows: given
a function computed by a marble transducer, can it be computed by a $k$-marble
transducer?  An easy lower bound is given by the size of the output, since for
instance we cannot produce a string of size $\Omega(n^2)$ with a two-way
transducer.  As shown in our third main result, it is in fact a sufficient
criterion to decide membership: a function from our class is computable with $k$
marbles if and only if it grows in $\mc{O}(n^{k+1})$ (and this property is
decidable).  This result shows the robustness of our $k$-marble model, since
a simple syntactical restriction is sufficient to describe a semantical
property.  Its proof is the most involved of this paper; it uses the
correspondence with $\SSTs$.

Similar optimization results have recently been obtained in
\cite{lhote2020pebble} for the class of \emph{polyregular functions}, defined
using $k$-pebble transducers \cite{bojanczyk2018polyregular} (an extension of
$k$-marble).  Interestingly, their conclusion is very similar to ours, that is:
an output of size $\mc{O}(n^k)$ can always be produced using $k$ nested loops.
We shall discuss in conclusion how our results both refine and extend theirs.
Contrary to us, the equivalence problem is an open problem for their model.
Furthermore, pebble transducers have never been related to a class of streaming
algorithms, contrary to what we show for marbles.


\subparagraph*{Outline.} After recalling in Section \ref{sec:prelim} the basic
definitions of two-way transducers and $\SSTs$, we present in Section
\ref{sec:marbles} the model of marble transducer and show equivalence.  We then
study in Section \ref{sec:bounded} the case of $k$-marble transducers and relate
them to specific $\SSTs$.  Finally, we solve in Section \ref{sec:membership} the
class membership problems associated with these models.  Due to space
constraints, several proofs are only sketched; we chose to focus on the proofs
of the last section since they describe an algorithm for program optimization.


==> Marbles arXiv/parts/marblesSST.tex <==
\label{sec:marbles}

As evoked in the introduction, our first goal is to extend Theorem
\ref{theo:alur} by describing a machine without registers that captures the
expressiveness of $\SSTs$ with copies.  For this purpose, we shall use a variant
of two-way transducers that can drop/lift several marks on their input.
However, the use of marks has to be strongly restricted so that the machine is
not too expressive (see e.g. \cite{ibarra1971characterizations}).  The model we
propose here, named \emph{marble transducer} after \cite{engelfriet1999trips},
can drop marks ("marbles") of different colors and the reading head has to stay 
on the left of marbles:
% only on the right of its reading head.  In other words, 
a stack of marks is stored on the % rightmost part of the
input and if the machine wants to move forward from a position where there is a
marble, it first has to remove it.


\begin{definition} \label{def:manymarbles}

A \emph{(deterministic) marble transducer} $\trans = (A,B,Q,C,q_0,\delta,\lambda,F)$ consists of:

\item 


\begin{itemize}

\item an input alphabet $A$;

\item a finite set of states $Q$ with an initial state $q_0 \in Q$ and a set $F \subseteq Q$ of final states;

\item a finite set of marble colors $C$;

\item a transition function $\delta: Q \times (A \uplus \{\lmark, \rmark\}) \times (C \uplus \{\varnothing\}) \rightarrow Q \times (\{\lmove, \rmove, \lift\} \uplus \{\drop_c\mid c \in C\})$ such that $\forall q\in Q, a \in A, c \in C$ we have $\delta(q,a,c) \in Q \times \{ \lmove,\lift \}$ (we cannot move right nor drop another marble when we see a marble).

\item an output function $\lambda: Q \times (A \uplus \{\lmark, \rmark\}) \times (C \uplus \{\varnothing\})  \rightarrow B^*$ with same domain as $\delta$.

\end{itemize}

\end{definition}

As for two-way transducers, the symbols $\lmark$ and $\rmark$ are used to denote
the borders of the input.  A \emph{configuration} over $\lmark w \rmark$ is a
tuple $(q,m, \pi)$ where $q \in Q$ is the current state, $m$ is the position of
the reading head, and $\pi = (c_{\ell},m_{\ell}) \cdots (c_1,m_1)$ is the stack
of the positions and colors of the $\ell$ marbles dropped (hence $\ell\geq0$ and
$0 \le m \le m_{\ell} < \cdots < m_1 \le |w|+1$ and $c_i \in C$).  An example of
configuration is depicted in Figure \ref{fig:config} below.


\begin{figure}[h!]

\begin{center}
\begin{tikzpicture}[scale=1]
	\node (in) at (-2.3,0) [right]{\small Input word};
	\fill[fill = blue,even odd rule] (2,0.5) circle (0.2);
	\fill[fill = red,even odd rule] (4,0.5) circle (0.2);
	\fill[fill = blue,even odd rule] (5,0.5) circle (0.2);
	\node[above] (in) at (0,-0.25) []{  $\lmark$};
	\node[above] (in) at (1,-0.25) []{  $b$};
	\node[above] (in) at (2,-0.25) []{  $a$};
	\node[above] (in) at (3,-0.25) []{  $b$};
	\node[above] (in) at (4,-0.25) []{  $b$};
	\node[above] (in) at (5,-0.25) []{  $b$};
	\node[above] (in) at (6,-0.25) []{  $a$};
	\node[above] (in) at (7,-0.25) []{  $\rmark$};
	\draw[](1.5,-0.5) rectangle (2.5,1);
        \draw[-](2,-0.5) to[out= -90, in = 90] (4,-1.25);
        	\node (in) at (2,1.25) []{\small Reading head};
	\node (in) at (3.9,-1.4) []{\small Control state $q$};
       \end{tikzpicture}
\end{center}

\vspace*{-0.3cm}
\caption{\label{fig:config} Configuration $(q, 2, (\textcolor{blue}{\bullet}, 2) (\textcolor{red}{\bullet}, 5) (\textcolor{blue}{\bullet}, 6))$ of a marble transducer over $babbba$. Note that allowed transitions starting from this configuration are either $\lift$ or $\lmove$.}

\end{figure}


The \label{mark:transrel} \emph{transition relation} $\rightarrow$ of $\trans$ is defined as follows. Given a configuration $(q,m, \pi)$, let $k := c$ if $\pi = (c,m) \cdots$ (marble $c$ in position $m$) and $k := \varnothing$ otherwise (no marble in $m$). Let $(q',\star):= \delta(q,w[m], k)$. Then $(q, m, \pi) \rightarrow (q', m', \pi')$ whenever one of the following holds:
\begin{itemize}

\item move left: $\star = \lmove$,  $m' = m-1 \ge 0$ and $\pi = \pi'$;

\item move right: $\star = \rmove$, $m' = m+1 \le |w|+1$ and $\pi = \pi'$ (only when $k = \varnothing$);

\item lift a pebble:  $\star = \lift$, $m = m'$ and $\pi = (c,m) \pi' $  (only when $k \neq \varnothing$);

\item drop a pebble: $\star = \drop_c$, $m = m'$, $\pi' = (c,m) \pi $  (only when $k = \varnothing$).

\end{itemize}
The notion of \emph{run} is defined as usual with $\rightarrow$. Accepting runs are finite runs that begin in $(q_0, 0, \varepsilon)$ and end in a configuration of the form $(q, |w|+1, \varepsilon)$ with $q \in F$.

The partial function $f : A^* \rightarrow B^*$ computed by the machine is defined as follows. If there exists an accepting run on $\lmark w \rmark$, then it is unique and $f(w)$ is the concatenation of all  the $\lambda(q,w[m], k)$ along the transitions of this run. Otherwise $f(w)$ is undefined.


\begin{remark} In case no marbles are used, the machine is simply a two-way transducer.
\end{remark}


As they can have an exponential number of configurations, marble transducers can
produce outputs of exponential size, like $\SSTs$ (see Example \ref{ex:expo:mt}).

\begin{example} \label{ex:expo:mt} 
  The function $\pow : a^n \mapsto a^{2^n}$ of Example \ref{ex:pow} is computed
  by a marble transducer with $C = \{0,1 \}$.  The idea is to use marbles to
  count in binary on the input $a^n$.  We first write $0^n$ on the input, then
  we increment it to $1{0}^{n-1}$, then $010^{n-2}$, $110^{n-2}$, $\dots$, $1^n$
  (there are $2^n$ numbers).  These increments can be done while preserving the
  stack discipline of the marbles: we move right and lift while we see
  $1$'s, when a $0$ is met we replace it by $1$, then we move left dropping
  $0$'s.  Initially and after each increment, we output an $a$ to produce $a^{2^n}$.
\end{example}


We are now ready to state our first generalization of Theorem \ref{theo:alur}. For the complexity, the size of a marble transducer is that of its output labels plus its number of marbles.

\begin{theorem} \label{theo:sstmt}
  Marble transducers and $\SSTs$ describe the same class of functions.  The
  right to left conversion is effective in $\PTIME$, and the converse one in
  $\EXP$.
\end{theorem}

\begin{proof}[Proof sketch.]  Let $\trans = (A,B,Q, C,q_0,\delta, \lambda,F)$ be
a marble transducer.  We simulate it with an $\SST$ by adapting the classical
reduction from two-way automata to one-way automata via \emph{crossing
sequences} \cite{shepherdson1959reduction}.  When in position $m$ of input $w
\in A^*$, the $\SST$ keeps track of the right-to-right runs of the marble
transducer on the prefix $w[1{:}m]$.  This abstraction is updated at each new
letter by considering the transitions it induces.  Due to the presence of
marbles, the same right-to-right run can be executed multiple times, but with
different stack of marbles (thus avoiding looping behaviors).  These multiple
similar executions are handled using copies in the $\SST$ model.  From $\SSTs$ to
marble transducers, we execute a recursive algorithm to compute the contents of
the registers, and implement it with a marble transducer using the marbles to
code the stack of calls (recursive calls are done from right to left, which
corresponds to the orientation of the marble stack).
\end{proof}

\begin{remark} Considering the domains, we note that marble automata
(transducers without the output) recognize exactly regular languages.  Indeed an
$\SST$ is easily seen to have a regular domain, since it is an extended one-way
automaton.  See \cite{engelfriet1999trips} for another proof of this fact.

\end{remark}


==> Marbles arXiv/parts/membership.tex <==
\label{sec:membership}

It is clear that a $k$-marble transducer is a particular case of $(k+1)$-marble transducer, which is a particular case of marble transducer (without restrictions). In other words, the classes of functions they define are included in each other. More precisely, these classes describe a strict hierarchy of increasing expressiveness, since $k$-marble transducers can only describe functions such that $|f(w)| = \mc{O}(|w|^{k+1})$ (see Examples \ref{ex:expo:mt} and \ref{ex:hierarchy} for  separation).

\begin{example} \label{ex:hierarchy} 
  The function $\powo^k: a^{n} \mapsto a^{n^k}$ can be computed with $k$
  marbles, but not less (since $|\powo^k(w)|$ is $\Omega(|w|^{k})$).  Let us
  explain the computation of $\powo^2$ with $1$ marble on input $a^n$.  We first
  drop the marble on position $n-1$, go to $1$, and move forward from $1$ to
  $n-1$ while outputting $aa$ at each transition.  Then we lift the marble and
  drop it on $n-2$, and perform the same outputs from $1$ to $n-2$, etc.  At the
  end of this procedure, we have output $a^{2((n-1)+ \cdots + 1)} = a^{n^2 -
  n}$.  It remains to output $a^n$ by reading the input once.
\end{example}

\begin{remark} Generalizing the construction of Example \ref{ex:hierarchy}, we can show that if $P \in \mb{N}[X]$ is a polynomial of degree $k \ge 0$, then $a^n \mapsto a^{P(n)}$ is computable with $k$ marbles (but not less).

\end{remark}

A natural problem when considering a hierarchy is that of \emph{membership}: given a function in some class, does it belong to a smaller one? The objective of this section is to provide a positive answer by showing Theorem \ref{theo:membership} below.

\begin{theorem} \label{theo:membership} Given a function $f$ described by a marble transducer, it is decidable in $\EXP$ whether $f$ can be computed by a $k$-marble transducer for some $k \ge 0$. In that case, we can compute the least possible $k \ge 0$ and build a $k$-marble transducer for $f$.
\end{theorem}

Proposition \ref{prop:growth} below is the key element for the proof, and is also interesting in itself. Indeed, it states that \emph{a polynomial-growth function can always be computed in polynomial time!} In other words, $f$ described by a marble transducer is computable with $k$ marbles if and only if $|f(w)| = \mc{O}(|w|^{k+1})$. Given $f : A^* \rightarrow B^*$, let $|f| : A^* \rightarrow \mb{N}, w \mapsto |f(w)|$.

\begin{definition} \label{def:growth}Let $g : A^* \rightarrow \mb{N}$, we say that $g$ has:
\begin{itemize}
\item \emph{exponential growth}, if $g(w) = \mc{O}(2^{\mc{O}(|w|)})$ and there exists an infinite set $L \subseteq A^*$ such that $g(w)= 2^{\Omega(|w|)}$ when $w \in L$;
\item \emph{$k$-polynomial growth} for $k \ge 0$, if $g(w) = \mc{O}(|w|^k)$ and there exists an infinite set $L \subseteq A^*$ such that $g(w) = \Omega(|w|^k)$ when $w \in L$;
\end{itemize}

\end{definition}

\begin{proposition} \label{prop:growth} Let $f : A^* \rightarrow B^*$ be a total function computed by a marble transducer. Then exactly one of the following is true:
\begin{itemize}
\item $|f|$ has exponential growth, and $f$ is not computable with $k$ marbles for any $k \ge 0$;
\item $|f|$ has $(k+1)$-polynomial growth for some $k \ge 0$, and $f$ is computable with $k$ marbles and $k$ is the least possible number of marbles;
\item $|f|$ has $0$-polynomial growth (i.e. a finite image), and $f$ is computable with $0$ marbles.
\end{itemize}
Moreover, these three properties are decidable in $\EXP$.
\end{proposition}

\begin{remark} If $f$ has a finite image, it is a trivial "step function": $\dom(f)$ is a finite union $ \bigcup_{i} L_i$ of regular languages such that $f$ is constant on each $L_i$.

\end{remark}

The rest of this section is devoted to the proof of these results.  By Theorem
\ref{theo:sstmt}, we first convert our marble transducer in an $\SST$ (in
$\EXP$), and only reason about $\SSTs$ in the sequel.  In fact, considering
$\SSTs$ is crucial: contrary to a marble transducer, an $\SST$ performs only one
pass on its input, which makes it possible to apply pumping-like arguments for
understanding the asymptotic growth of the outputs.  Some proof techniques used
below are inspired from \cite{filiot2017copyful} which only considers deciding
$1$-polynomial growth of $\SSTs$.

\subsection{Simplification of $\SST$}

An $\SST$ is said to be \emph{total} whenever its transition, update and output functions are total. We shall assume that our machine is so. Indeed, it can be completed like a finite automaton, by outputting $\varepsilon$ when out of the domain. Furthermore, this operation does not modify the asymptotic growth of the computed function.

We say that an $\SST$ is \emph{simple} if it is total, it has a single state (i.e. $Q = \{q_0\}$), and its substitutions and output do not use letters (i.e. $\lambda : Q \times A \rightarrow \subst{\regs}{\varnothing}$ and $F:Q \rightarrow \regs^*$). 
To simplify the notations, we write $(A,B, \regs, \iota, \lambda, F)$ for a
simple $\SST$, where $\lambda: A \rightarrow \subst{\regs}{\varnothing}$ and $F
\in \regs^*$.  Indeed, states and the transition function are useless.


\begin{lemma} \label{lem:simple} Given a total $\SST$, we can build an equivalent simple $\SST$ in $\PTIME$.
\end{lemma}

\begin{proof}[Proof.] 
  Let $\trans = (A,B,Q, \regs, q_0, \iota, \delta, \lambda, F)$ be the original
  $\SST$.  We can assume that it uses no letters in the substitutions by storing
  them in constant registers (using the initial function).  To remove the
  states, we let $\regs' := Q \times \regs$ be our new register set.  In our new
  machine, register $(q,x)$ will contain the value of $x$ if $q$ is the current
  state of $\trans$, and $\varepsilon$ otherwise.  The update function $\lambda'
  : A \rightarrow \subst{\regs'}{B}$ and output $F' \in \regs'^*$ are defined as
  follows:
  $$
  \lambda'(a)(q,x) = \prod_{p \mid \delta(p,a) = q} \mu_{p}(\lambda(p,a)(x)) \text{ and } F' =  \prod_{q \in \dom(F)} \mu_{p}(F(q))
  $$
  where $\mu_p$ replaces $y \in \regs$ by $(p,y) \in \regs'$. During a run, at most one term of the concatenation defining $\lambda'(a)(q,x)$ is nonempty, the one which corresponds to the true state $p$ of $\trans$. 
\end{proof}

\begin{remark} However, this construction does not preserve copylessness nor $k$-layeredness.
\end{remark}


\subsection{Asymptotic behavior of $\mb{N}$-automata and $\SSTs$}

Given a simple $\SST$, we first build an $\mb{N}$-automaton that "computes" the
size of the words stored in the registers along a run of the $\SST$.  As we
shall see, the growth of functions produced by $\mb{N}$-automata exactly matches
the case disjunction of Proposition \ref{prop:growth}.

\begin{definition} \label{def:naut} An $\mb{N}$-automaton $\auto = (A,\staa,\inia,\weia,\fina)$ consists in:

\item

\begin{itemize}

\item an input alphabet $A$;

\item a finite set $\staa$ of states;

\item an initial row vector $\inia \in \mb{N}^{\staa}$ and a final column vector $\fina \in \mb{N}^{\staa}$;

\item a monoid morphism $\weia : A^* \rightarrow \mb{N}^{\staa \times \staa}$ (weight function).

\end{itemize}

\end{definition}

The automaton $\auto$ computes the total function $ A^* \rightarrow \mb{N}, w \mapsto \inia \weia(w) \fina$. We say that it is \emph{trim} if $\forall q \in \staa$, $\exists u,v \in A^*$ such that $(\inia \weia(u))(q) \ge 1$ and $(\weia(v)\fina)(q) \ge 1$.


Let $ \trans =(A,B, \regs, \iota, \lambda, F)$ be a simple $\SST$, we define its
\emph{flow automaton} $\fauto{\trans} := (A, \regs, \inia,\weia,\fina)$ as the
$\mb{N}$-automaton with input $A$, states $\regs$, and:
\begin{itemize}
\item for all $x \in \regs$, $\inia(x) = |\iota(x)|$ (number of letters initialized in $x$);

\item for all $x \in \regs$, $\fina(x)$ is the number of occurrences of $x$ in $F$;

\item for all $a \in A, x,x' \in \regs$, $\weia(a)(x,x')$ is the number of occurrences of $x$ in $\lambda(a)(x')$.
\end{itemize}

Recall that $\trans^{w}(x)$ is "the value of $x$ after reading $w$ in $\trans$"; the flow automaton indeed computes the size of these values. We get the following by induction.

\begin{claim} \label{claim:nauto} For all $w \in A^*$ and $x \in \regs$, we have $(\inia \weia(w))(x) = |\trans^{w}(x)|$. In particular, if $f$ is the function computed by $\trans$, then $\fauto{\trans}$ computes $|f|$.
\end{claim}


Without loss of generality, we can assume that $\fauto{\trans}$ is trim. Indeed, if $x \in \regs$ is such that $(\inia \weia(u))(x) = 0$ for all $u \in A^*$, then $x$ always has  value $\varepsilon$ and can be erased everywhere in $\trans$. Similarly, if $(\weia(v)\fina)(x) = 0$ for all $v \in A^*$, $x$ is never used in the output.

Let us now study in detail the asymptotic behavior of $\mb{N}$-automata.

\begin{lemma} \label{lem:graph} Let $\auto = (A, \staa, \inia, \weia,\fina)$ be a trim $\mb{N}$-automaton that computes a function $g:A^* \rightarrow \mb{N}$. Then one of the following holds, and it can be decided in $\PTIME$:

\item 

\begin{itemize}

\item \label{po:bound} $g$ has an exponential growth;

\item \label{po:partition} $g$ has $k$-polynomial growth for some $k \ge 0$ and $\staa = \biguplus_{0 \le i \le k} S_i $ is such that:
\begin{itemize}

\item $\forall q,q' \in \staa$, if $\exists w \in A^*$ such that 
$\weia(w)(q,q') \ge 1$ then $q \in S_i, q'\in S_{j}$ for some $i \le j$;

\item $\exists B \ge 0$ such that $\forall 0 \le i \le k$, $\forall q,q' \in S_i, \forall w \in A^*$, $\weia(w)(q,q') \le B$;

\item $\forall q \in S_i, (\inia \weia(w))(q) = \mc{O}(|w|^i)$.

\end{itemize}

\end{itemize}

Furthermore, $k$ and $S_0, \dots, S_k$ are computable in $\PTIME$.

\end{lemma}



\begin{remark} An upper bound $B$ can be described explicitly, see e.g. \cite{sakarovitch2008decidability}.

\end{remark}




\begin{proof}[Proof sktech.] Very similar results are obtained in \cite{weber1991degree} for computing ambiguity of finite automata (which corresponds to $\mb{N}$-automata with weights in $\{0,1\}$ only).  However, in order to keep the paper self-contained, we give a detailed proof  in Appendix.

Mainly, we look for the presence of the two patterns from \cite{sakarovitch2008decidability} in the weights of $\auto$:
\begin{itemize}

\item \emph{heavy cycles} ($\exists q \in \staa, v \in A^*$ such that $\weia(v)(q,q) \ge 2$), that creates exponential growth ;

\item  \emph{barbells} ($\exists q \neq q', v \in A^{+}$, such that $\weia(v)(q,q)  \ge 1$, $\weia(v)(q,q')  \ge 1$ and $\weia(v)(q',q')  \ge 1$) such that a chain of $k$ barbells induces $k$-polynomial growth.
\end{itemize}
\vspace*{-1\baselineskip}
\end{proof}

As a consequence, if $f$ is computed by an $\SST$, then $|f|$ has either exponential growth or $k$-polynomial growth for some $k \ge 0$. Furthermore, we can decide it in $\PTIME$.

It remains to show that if $|f|$ has a $(k+1)$-polynomial growth, then $f$ is computable by a $k$-layered $\SST$. For this, we shall use the partition of Lemma \ref{lem:graph} that splits the simple $\SST$ (via the states of its flow automaton) in a somehow $k$-layered way. However, the layers obtained are not directly copyless, and another transformation is necessary.









\subsection{Construction of $k$-layered $\SST$ in the polynomial case}


If $|f|$ has $(k+1)$-polynomial growth, then Lemma \ref{lem:graph} partitions
the simple $\SST$ in $k+2$ layers.  Our first concern is to get $k+1$ layers
only, since we want a $k$-layered $\SST$.  In the next definition,
$\lambda(p,w)$ denotes the substitution applied when reading $w \in A^*$ from
$p\in Q$, that is $\lambda(p,w[1]) \circ \cdots
\lambda(\delta(p,w[1{:}(i-1)]),w[i]) \circ \cdots \circ
\lambda(\delta(p,w[1{:}(|w|-1)]),w[|w|])$.

\begin{definition} \label{def:bounded} 
  We say that an $\SST$ $(A, B, Q, \regs, q_0, \iota, \delta, \lambda, F)$ is
  \emph{$(k,B)$-bounded} if there exists a partition $\regs_0,\regs_1, \dots,
  \regs_k$ of $\regs $ such that $\forall q \in Q, a \in A, w \in A^*$:
  \begin{itemize}
    \item $\forall 0 \le i \le k$, only registers from $\regs_0, \dots, \regs_i$ appear in $\{\lambda(q,a)(x) \mid {x \in \regs_i}\}$;
    \item $\forall 0 \le i \le k$, each $y \in \regs_i$ appears at most
    $B$ times in $\{\lambda(q,w)(x) \mid x \in \regs_i\}$.
  \end{itemize}
\end{definition}


For $k=0$, Definition \ref{def:bounded} means that at most $B$ copies of $y$ are "useful" during a run.  The $(0,B)$-bounded $\SSTs$ are known as \emph{$B$-bounded (copy) $\SSTs$}
in \cite{dartois2016aperiodic} (however, contrary to what is said in
\cite{dartois2016aperiodic,filiot2017copyful}, it is not the same definition as
the "bounded copy" of \cite{alur2012regular}). For some $k \ge 1$, a $(k,B)$-bounded $\SST$ is similar to a $k$-layered $\SST$, except that each layer is no longer "copyless in itself" but "$B$-bounded in itself". In particular, we note that $(k,1)$-bounded $\SSTs$ exactly correspond to $k$-layered $\SSTs$.



\begin{lemma} \label{lem:boundedcopy} 
  Given a simple $\SST$ that computes a function $f$ such that $|f|$ has
  $(k+1)$-polynomial growth, we can build an equivalent $(k,B)$-bounded $\SST$ for
  some $B \ge 0$.
\end{lemma}

\begin{proof}[Proof sketch.] Let $S_0, \dots, S_{k+1}$ be the partition of the registers given by Lemma \ref{lem:graph}. During a run, note that the registers in $S_0$ can only store strings of a bounded size. The idea is to remove $S_0$ and hardcode the content of each $x \in S_0$ in  a finite set of states. The transition function is defined following their former updates. The new update function is defined by replacing the mention of $x \in S_0$ by its explicit content (given by the current state).
\end{proof}


\begin{remark} As for weighted automata above, an upper bound $B$ can effectively be computed.
\end{remark}

It is known that a $(0,B)$-bounded $\SST$ can be transformed in a copyless $\SST$. The proof requires rather complex constructions, that we generalize for a $(k,B)$-bounded $\SST$.



\begin{lemma} \label{lem:kbounded} Given a $(k,B)$-bounded $\SST$, we can build an equivalent $k$-layered $\SST$.
\end{lemma}

\begin{proof}[Proof sketch.] The proof is done by induction on $k \ge 0$. Indeed a $(k,B)$-bounded (resp. $k$-layered) $\SST$ is somehow a $B$-bounded (resp. copyless) $\SST$, that can also "call" registers from the lower layers. Hence we only need to focus on transforming \emph{one} layer. The difficulty is to take into account copies coming from the lower layers. This is done by introducing an intermediate model of \emph{$\SST$ with external functions} ($\SSTF$), which corresponds to an $\SST$ with a set of functions $\oras$ that can be called in an oracle-like style.

Thus our proof roughly consists in showing that a $B$-bounded $\SSTF$ (in the sense of Definition \ref{def:bounded}) can be transformed in a copyless $\SSTF$. This is done in two steps. First, we transform the $B$-bounded $\SSTF$ in a copyless \emph{non-deterministic} $\SSTF$, following the ideas of \cite{dartois2016aperiodic} for $\SST$. Non-deterministic transducers usually compute relations between words, but we in fact obtain an \emph{unambiguous} machine (i.e. that has at most one accepting run on each input), hence describing a function. Second, we show that a copyless unambiguous non-deterministic $\SSTF$ can be converted in a copyless $\SSTF$. This transformation relies on the techniques of \cite{alur2012regular} (developped for $\SST$ over infinite words).
\end{proof}

\begin{proof}[Proof of Theorem \ref{theo:membership}.] 
We first transform an $\SST$ into a simple $\SST$ (Lemma \ref{lem:simple}) and build its flow automaton. Using this machine, one can decide what is the growth of $|f|$ (Lemma \ref{lem:graph}). If $|f|$ has $(k+1)$-polynomial growth, we then build a $(k,B)$-bounded $\SST$ that computes it (Lemma \ref{lem:boundedcopy}) and finally a $k$-layered $\SST$ (Lemma \ref{lem:kbounded}).
\end{proof}






==> Marbles arXiv/parts/preliminaries.tex <==
\label{sec:prelim}


We denote by $\mb{N}$ the set of nonnegative integers. Capital letters $A$ and $B$ are used to denote alphabets, i.e. finite sets of letters. If $w \in A^*$ is a word, let $|w| \in\mb{N}$ be its length, and for $1 \le m \le |w|$ let $w[m]$ be its $m$-th letter. The empty word is denoted $\vide$. If $1 \le m \le n \le |w|$, let $w[m{:}n] = w[m]w[m+1] \cdots w[n]$. We assume that the reader is familiar with the basics of automata theory, and in particular the notions of one-way and two-way deterministic automata (see e.g. \cite{shepherdson1959reduction}).

\subparagraph*{Two-way transducers.} A deterministic two-way transducer is a deterministic two-way automaton enhanced with the ability to produce outputs along its run.  The class of functions described by these machines is known as "regular functions" \cite{chytil1977serial, engelfriet2001mso}.


\begin{definition} A \emph{(deterministic) two-way transducer} $\trans = (A,B,Q,q_0, \delta, \lambda,F)$ consists of:
\begin{itemize}
\item an input alphabet $A$, an output alphabet $B$;
\item a finite set of states $Q$, with an initial state $q_0 \in Q$  and a set of final states $F \subseteq Q$ ;
\item a (partial) transition function $\delta: Q \times (A\uplus\{  \lmark,\rmark) \rightarrow Q \times \{\lmove, \rmove\}$;
\item a (partial) output function $\lambda: Q \times (A\uplus\{ \lmark,\rmark\} ) \rightarrow B^*$ with same domain as $\delta$.
\end{itemize}
\end{definition}


When given as input a word $w \in A^*$, the two-way transducer disposes of a read-only input tape containing $\lmark w \rmark$. The marks $\lmark$ and $\rmark$ are used to detect the borders of the tape, by convention we denote them as positions $0$ and $|w|+1$ of $w$.

Formally, a \emph{configuration} over  $\lmark w \rmark$ is a tuple $(q,m)$ where $q \in Q$ is the current state and $0 \le m \le |w|+1$ is the position of the reading head. The \emph{transition relation} $\rightarrow$ is defined as follows. Given a configuration $(q,m)$, let $(q',\star):= \delta(q,w[m])$. Then $(q, m) \rightarrow (q', m')$ whenever either $\star = \lmove$ and  $m' = m-1$ (move left), or $\star = \rmove$ and $m' = m+1$ (move right), with $0 \le m' \le |w|+1$. A \emph{run} is a sequence of configurations following $\rightarrow$. Accepting runs are those that begin in $(q_0, 0)$ and end in a configuration of the form $(q, |w|+1)$ with $q \in F$.

The (partial) function $f : A^* \rightarrow B^*$ computed by the machine is defined as follows. If there exists an accepting run on $\lmark w \rmark$, then it is unique and $f(w)$ is the concatenation of all  the $\lambda(q,w[m])$ along the transitions of this run. Otherwise $f(w)$ is undefined.

\begin{example} \label{ex:mirror} Let $\mirror : A^* \rightarrow A^*$ be the function that maps a word $abac$ to its mirror image $caba$. It can be performed by a two-way transducer that first goes to the right symbol $\rmark$, and then reads $w$ from right to left while outputting the letters.
\end{example}




\subparagraph*{Streaming string transducers.} Informally, a \emph{streaming
string transducer} \cite{alur2010expressiveness} is a one-way deterministic
automaton with a finite set $\regs$ of registers that store strings over the
output alphabet $B$.  These registers are modified using \emph{substitutions},
i.e. mappings $\regs \rightarrow (B \uplus \regs)^*$.  We denote by
$\subst{\regs}{B}$ the set of these substitutions.  They can be extended
morphically from $(B \uplus \regs)^*$ to $ (B \uplus \regs)^*$ by preserving the
elements of $B$.  As explained in Example \ref{ex:subst}, they can be composed
by setting $(s_1 \circ s_2)(x) := s_1 (s_2(x))$ for $x \in \regs$.





\begin{example} \label{ex:subst} Let $\regs = \{x,y\}$ and $B = \{b\}$. Consider the substitutions $s_1:= x \mapsto b, y \mapsto bxyb$ and $s_2:= x \mapsto xb, y \mapsto xy$, then $ s_1 \circ s_2 (x) = s_1(xb) = bb$ and $ s_1 \circ s_2 (y) = s_1(xy) = bbxyb$.
\end{example}

\begin{definition}A \emph{streaming string transducer} ($\SST$) $\trans = (A,B, Q,\regs,q_0, \iota, \delta, \lambda,F)$ is:
\begin{itemize}

\item an input alphabet $A$ and an output alphabet $B$;

\item a finite set of states $Q$ with an initial state $q_0 \in Q$;

\item a finite set $\regs$ of registers;

\item an initial function $\iota : \regs \rightarrow B^*$;

\item a (partial) transition function $\delta : Q \times A \rightarrow Q$;

\item a (partial) register update function $\lambda: Q \times A \rightarrow \subst{\regs}{B}$  with same domain as $\delta$;

\item a (partial) output function  $F: Q \rightarrow (\regs \cup B)^*$.

\end{itemize}
\end{definition}


This machine defines a (partial) function $f : A^* \rightarrow B^*$ as follows. Let us fix $w \in A^*$. If there is no accepting run of the \emph{one-way} automaton $(A, Q,q_0, \delta, \dom(F))$ over $w$, then $f(w)$ is undefined. Otherwise, let $q_m:= \delta(q_0,w[1{:}m])$ be the $m$-th state of this run. We define for $0 \le m \le |w|$, $\trans^{w[1{:}m]} \in \subst{\regs}{B}$ ("the values of the registers after reading $w[1{:}m]$") as follows:
\begin{itemize}

\item $\trans^{w[1:0]} (x) = \iota(x)$ for all $x \in \regs$; \label{mark:valu}

\item for $1 \le m \le |w|$, $\trans^{w[1{:}m]} := \trans^{w[1{:}(m-1)]}\circ\lambda(q_m, w[m])$. This formula e.g. means that if $\trans^{w[1{:}(m-1)]}(x) = ab$ and $\lambda(q_m, w[m])(x) = xx$, then $\trans^{w[1{:}m]}(x) = abab$.

\end{itemize}
In this case, we set $f(w) := \trans^{w}(F(q_{|w|})) \in B^*$. In other words, we combine the final values of the registers following the output function.

\begin{example} \label{ex:mirror:sst} 
  The $\mirror$ of Example \ref{ex:mirror} can be computed by an $\SST$ with
  one state and one register $x$.  When seeing a letter $a$, the $\SST$ updates
  $x\mapsto ax$ ($a$ is added in front of $x$).
\end{example}

\begin{example} \label{ex:pow} Consider the function $\pow:a^n \mapsto a^{2^n}$. It is computed by an $\SST$ with one register $x$ initialized to $a$ and updated $x \mapsto xx$ at each transition.
\end{example}

The function $\pow$ of Example \ref{ex:pow} cannot be computed by a
deterministic two-way transducer.  Indeed, a two-way transducer computing a
function $f$ has only $|Q|(|w|+2)$ possible configurations on input $w$,
therefore we must have $|f(w)| = \mc{O}(|w|)$.


In order to make two-way transducers and $\SSTs$ coincide, the solution of
\cite{alur2010expressiveness} is to forbid duplications of registers.  A
substitution $\sigma \in \subst{\regs}{B}$ is said to be \emph{copyless} if each
register $x \in \regs$ appears at most once in the whole set of words
$\{\sigma(x)\mid x \in \regs\}$.  The substitution $s_1$ of Example
\ref{ex:subst} is copyless whereas $s_2$ is not.  An $\SST$ is said to be copyless
whenever it uses only copyless substitutions for the $\lambda(q,a)$; the $\SST$
of Example \ref{ex:mirror:sst} is so.


\begin{theorem}[\cite{alur2010expressiveness, dartois2017reversible}] \label{theo:alur} 
  Two-way transducers and copyless $\SSTs$ describe the same class of functions
  ("regular functions").  The right to left conversion is effective in $\PTIME$,
  and the converse one in $\EXP$.
\end{theorem}


\begin{remark}
For the complexities, the "size" of the machines is that of a reasonable representation. For a two-way transducer, it is roughly the total size of the outputs that label its transitions. For an $\SST$, it is the total size of its substitutions.
\end{remark}


















